Understanding Pure CLIP Guidance for Voxel Grid NeRF Models

We explore the task of text to 3D object generation using CLIP. Specifically, we use CLIP for guidance without access to any datasets, a setting we refer to as pure CLIP guidance. While prior work has adopted this setting, there is no systematic study of mechanics for preventing adversarial generations within CLIP. We illustrate how different image-based augmentations prevent the adversarial generation problem, and how the generated results are impacted. We test different CLIP model architectures and show that ensembling different models for guidance can prevent adversarial generations within bigger models and generate sharper results. Furthermore, we implement an implicit voxel grid model to show how neural networks provide an additional layer of regularization, resulting in better geometrical structure and coherency of generated objects. Compared to prior work, we achieve more coherent results with higher memory efficiency and faster training speeds.

==> Figures/tex/Fig-Ensemble.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{Figures/source/Fig-Ensemble.pdf}
\caption{Generation results using different ensembles of the various CLIP models.}
\label{fig:Ensemble}
\end{figure*}


==> Figures/tex/Fig-Failure.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{Figures/source/Fig-Failure.pdf}
\caption{Multi-view images of the objects generated from the input text prompts. Although the textures resembles what is described by the prompt from some views, the geometry is incorrect for actual object in the real world.}
\label{fig:Failure}
\end{figure*}

